On the radio spectra of Galactic millisecond pulsars

With recent advances in the sensitivity of radio surveys of the Galactic disk, the number of millisecond pulsars (MSPs) has increased substantially in recent years such that it is now possible to study their demographic properties in more detail than in the past. We investigate what can be learned about the radio spectra of the MSP population. Using a sample of 179 MSPs detected in eleven surveys carried out at radio frequencies in the range 0.135-6.6 GHz, we carry out detailed modeling of MSP radio spectral behaviour in this range. Employing Markov Chain Monte Carlo simulations to explore a multi-dimensional parameter space, and accurately accounting for observational selection effects, we find strong evidence in favour of the MSP population having a two-component power-law spectral model scaling with frequency, $\nu$. Specifically, we find that MSP flux density spectra are approximately independent of frequency below 320 MHz, and proportional to $\nu^{-1.5}$ at higher frequencies. This parameterization performs significantly better than single power-law models which over predict the number of MSPs seen in low-frequency (100-200 MHz) surveys. We compared our results with earlier work, and current understanding of the normal pulsar population, and use our model to make predictions for MSP yields in upcoming surveys. We demonstrate that the observed sample of MSPs could triple in the coming decade.

==> converged_parameter_table.tex <==
\begin{table}
\caption{Converged parameters obtained using MCMC for each model. Values without errors were kept constant during the MCMC. Different alphabets represent different models as explained in section 4. For model g, h, i, two spectral indexes were used with a break frequency. The first value is the high frequency spectral index, and the second value is lower frequency spectral index.}
\centering
\label{tab:converged_parameters}
\begin{tabular}{lccccccc}
\hline \hline
% \noalign{\smallskip} \hline \hline \noalign
Model & $\mu_{SI}$ & $\sigma_{SI}$ & $z_{0}$ & $<\log$L$>$ & $\sigma(\log$L)  & Break Freq (MHz) & Metric \\
\hline
A & -1.3$^{+0.19}_{-0.22}$ & 0.43$^{+0.33}_{-0.28}$ & 0.5 & -1.1 & 0.9& - & 3.6$^{+1.4}_{1.19}$ \\
\hline
B & -0.99$^{+0.2}_{-0.25}$ & 0.7 & 0.91$^{+0.34}_{-0.29}$ & -1.1 & 0.9& - & 3.24$^{+1.6}_{1.26}$ \\
\hline
C & -1.19$^{+0.33}_{-0.45}$ & 0.7 & 0.9$^{+0.33}_{-0.27}$ & -0.78$^{+0.35}_{-0.49}$ & 0.9& - & 3.04$^{+1.16}_{1.11}$ \\
\hline
D & -1.47$^{+0.27}_{-0.3}$ 0.26$^{+1.01}_{-0.82}$ & 0.7 & 0.5 & -1.1 & 0.9& 301.13$^{+122.06}_{-65.4}$ & 1.28$^{+0.72}_{0.46}$ \\
\hline
E & -1.53$^{+0.21}_{-0.27}$ -0.05$^{+0.64}_{-0.61}$ & 0.7 & 0.5 & -1.1 & 0.9& 400 & 1.77$^{+1.31}_{0.57}$ \\
\hline
\end{tabular}
\end{table}

==> results_table.tex <==
\begin{table*}
\caption{Table showing the median number of MSPs discovered in the surveys (with one sigma) obtained by running the simulations 100 times at the converged parameter values obtained using MCMC.}
\centering
\label{tab:hundred_run_results}
\begin{tabular}{lcrrrrrr}
    % \noalign{\smallskip} 
    \hline \hline 
    % \noalign
    Survey & Freq. (MHz) & N & A &  B & C & D & E \\
    \hline
    LOTAAS & 135 & 10 & 22$^{+4}_{-5}$ & 21$^{+4}_{-4}$ & 20$^{+4}_{-4}$ & 10$^{+3}_{-3}$ & 10$^{+4}_{-3}$\\
    \hline
    AODRIFT & 327 & 33 & 22$^{+4}_{-4}$ & 25$^{+5}_{-4}$ & 24$^{+5}_{-4}$ & 38$^{+4}_{-6}$ & 23$^{+4}_{-4}$\\
    \hline
    GBNCC & 350 & 61 & 58$^{+4}_{-6}$ & 59$^{+5}_{-4}$ & 62$^{+4}_{-6}$ & 64$^{+5}_{-6}$ & 65$^{+5}_{-5}$\\
    \hline
    PKS70 & 436 & 19 & 16$^{+4}_{-3}$ & 16$^{+3}_{-3}$ & 18$^{+4}_{-3}$ & 18$^{+4}_{-4}$ & 22$^{+4}_{-3}$\\
    \hline
    DMB & 1374 & 2 & 2$^{+1}_{-2}$ & 1$^{+1}_{-1}$ & 1$^{+1}_{-1}$ & 1$^{+2}_{-1}$ & 2$^{+1}_{-1}$\\
    \hline
    PHSURV & 1374 & 5 & 4$^{+3}_{-2}$ & 4$^{+2}_{-2}$ & 3$^{+2}_{-1}$ & 4$^{+1}_{-2}$ & 4$^{+2}_{-2}$\\
    \hline
    PASURV & 1374 & 1 & 3$^{+2}_{-2}$ & 2$^{+2}_{-1}$ & 2$^{+1}_{-1}$ & 2$^{+2}_{-1}$ & 3$^{+2}_{-2}$\\
    \hline
    PMSURV & 1374 & 28 & 28$^{+5}_{-5}$ & 21$^{+5}_{-3}$ & 22$^{+5}_{-6}$ & 24$^{+4}_{-6}$ & 27$^{+7}_{-4}$\\
    \hline
    SWINHL & 1374 & 8 & 10$^{+3}_{-3}$ & 13$^{+3}_{-4}$ & 13$^{+3}_{-4}$ & 8$^{+2}_{-2}$ & 9$^{+3}_{-3}$\\
    \hline
    SWINIL & 1374 & 12 & 14$^{+3}_{-4}$ & 14$^{+3}_{-3}$ & 15$^{+3}_{-4}$ & 11$^{+3}_{-4}$ & 13$^{+2}_{-3}$\\
    \hline
    MMB & 6600 & 0 & 0$^{+1}_{-0}$ & 1$^{+0}_{-1}$ & 0$^{+1}_{-0}$ & 0$^{+1}_{-0}$ & 0$^{+1}_{-0}$\\
    \hline
    %  & Total & 179 & 3.6$^{+1.4}_{-1.19}$ & 3.24$^{+1.6}_{-1.26}$ & 3.04$^{+1.16}_{-1.11}$ & 1.28$^{+0.72}_{-0.46}$ & 1.77$^{+1.31}_{-0.57}$ \\
    % \hline
    % \hline
    Metric & & & 3.6$^{+1.4}_{-1.19}$ & 3.24$^{+1.6}_{-1.26}$ & 3.04$^{+1.16}_{-1.11}$ & 1.28$^{+0.72}_{-0.46}$ & 1.77$^{+1.31}_{-0.57}$ \\
    \hline\hline
    % \bottomrule
\end{tabular}
\end{table*}
